Estimation of Video Streaming KQIs for Radio Access Negotiation in Network Slicing Scenarios

The use of multimedia content has hugely increased in recent times, becoming one of the most important services for the users of mobile networks. Consequently, network operators struggle to optimize their infrastructure to support the best video service-provision. As an additional challenge, 5G introduces the concept of network slicing as a new paradigm that presents a completely different view of the network configuration and optimization. A main challenge of this scheme is to establish which specific resources would provide the necessary quality of service for the users using the slice. To address this, the present work presents a complete framework for this support of the slice negotiation process through the estimation of the provided Video Streaming Key Quality Indicators (KQIs), which are calculated from network low-layer configuration parameters and metrics. The proposed estimator is then evaluated in a real cellular scenario.

==> IEEE_PAPER_PACKAGES.tex <==
\usepackage[latin1]{inputenc}
\usepackage[spanish, english]{babel}

%--------------------------------
%\usepackage{subcaption}


\usepackage{url}

\usepackage{graphics,graphicx} %paquetes grÃ¯Â¿Â½ficos estÃ¯Â¿Â½ndar%
\usepackage{wrapfig} %paquete para grÃ¯Â¿Â½fica lateral%
\usepackage[rflt]{floatflt} %figuras flotantes%
% \begin{floatingfigure}[r]/[l]{4.5cm}
% \end{floatingfigure}
\usepackage{graphpap}	%comando \graphpaper en el entorno picture%
\usepackage{graphicx}

\usepackage{tabularx} % in the preamble
\usepackage{multirow}

% https://tex.stackexchange.com/questions/166790/how-can-i-get-straight-double-quotes-in-listings
\usepackage{textcomp}
\usepackage{listings}
 % Para escribir piezas de cÃ¯Â¿Â½digo C, Python, etc. %
%listings configuration

\lstset{
	language=Python, %Puede ser C, C++, Java, etc.
	showstringspaces=false,
	formfeed=\newpage,
	tabsize=4,
	commentstyle=\itshape,
	basicstyle=\ttfamily,
	morekeywords={models, lambda, forms}
	%numberstyle=\tiny, 
	%breaklines=true,
	backgroundcolor=\color{white},
	%numbersep=5pt,
	xleftmargin=.35in,
	xrightmargin=.25in
}

\lstset{upquote=true, language=C}
\usepackage{xcolor}


\colorlet{punct}{red!60!black}
%\definecolor{background}{HTML}{EEEEEE}
\definecolor{background}{HTML}{FDFDFD}
\definecolor{delim}{RGB}{20,105,176}
\colorlet{numb}{magenta!60!black}

\lstdefinelanguage{json}{
	basicstyle=\normalfont\ttfamily,
	numbers=left,
	numberstyle=\scriptsize,
	stepnumber=1,
	numbersep=8pt,
	showstringspaces=false,
	breaklines=true,
	frame=single,
	backgroundcolor=\color{background},
	literate=
	*{0}{{{\color{numb}0}}}{1}
	{1}{{{\color{numb}1}}}{1}
	{2}{{{\color{numb}2}}}{1}
	{3}{{{\color{numb}3}}}{1}
	{4}{{{\color{numb}4}}}{1}
	{5}{{{\color{numb}5}}}{1}
	{6}{{{\color{numb}6}}}{1}
	{7}{{{\color{numb}7}}}{1}
	{8}{{{\color{numb}8}}}{1}
	{9}{{{\color{numb}9}}}{1}
	{:}{{{\color{punct}{:}}}}{1}
	{,}{{{\color{punct}{,}}}}{1}
	{\{}{{{\color{delim}{\{}}}}{1}
	{\}}{{{\color{delim}{\}}}}}{1}
	{[}{{{\color{delim}{[}}}}{1}
	{]}{{{\color{delim}{]}}}}{1},
}



%-------------------------------------------------------
\usepackage{adjustbox}
\usepackage{longtable}

\usepackage[english, plain]{fancyref} % plain, 
\fancyrefchangeprefix{\fancyreftablabelprefix}{table}
\newcommand*{\fancyrefpartlabelprefix}{part}
\fancyrefchangeprefix{\fancyrefpartlabelprefix}{part}



%\renewcommand*{\sectionname}{Sección}


\usepackage{enumitem}

%-----------------------------------------------------------
%\usepackage{pdfcomment}
%\defineavatar{SFR}{color={1 0 0},author={SFR}}%
%\usepackage[disable]{pdfcomment}
%
%
%\definestyle{MyStyle}{icon=Comment,opacity=0.6,voffset=8pt,hoffset=0.965\textwidth }% Less offset
%\definestyle{MyStyle2}{icon=Comment,opacity=0.6,voffset=8pt,hoffset=0.965\textwidth }%

%------------------------------------------------------------
\usepackage[parfill]{parskip}


%-----------------------------------
% https://www.sharelatex.com/blog/2013/02/16/using-latexdiff-for-marking-changes-to-tex-documents.html
%\usepackage[options]{trackchanges} 
%\addeditor{Sergio} 
%\addeditor{David} 
% https://www.sharelatex.com/blog/2013/02/16/using-latexdiff-for-marking-changes-to-tex-documents.html

%---------------------------------------------------------------------------------
%https://www.inf.ethz.ch/personal/markusp/teaching/guides/guide-tables.pdf
\usepackage{booktabs}

\newlength{\tpw}
\setlength{\tpw}{0.25ex} % top bar width

\newcommand\asta{1.3} % \renewcommand{\arraystretch}{1.2}


% Left
\newcolumntype{P}[1]{>{\RaggedRight\hspace{0pt}}p{#1}}
\newcolumntype{M}[1]{>{\RaggedRight\hspace{0pt}}m{#1}}

% Centered
\newcolumntype{Q}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}p{#1}}
\newcolumntype{N}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

% Right
\newcolumntype{R}[1]{>{\RaggedLeft\hspace{0pt}}p{#1}}
\newcolumntype{O}[1]{>{\RaggedLeft\hspace{0pt}}m{#1}}


%----------------------------------
%https://tex.stackexchange.com/questions/52351/quote-marks-are-backwards-using-texmaker-pdflatex
%\usepackage [autostyle, english = american]{csquotes}
%\MakeOuterQuote{"}

%https://tex.stackexchange.com/questions/7735/how-to-get-straight-quotation-marks
%\usepackage{upquote}
%https://tex.stackexchange.com/questions/59424/cant-include-pifont
%\usepackage{fonttable}


